BinPro: A Tool for Binary Source Code Provenance

Enforcing open source licenses such as the GNU General Public License (GPL), analyzing a binary for possible vulnerabilities, and code maintenance are all situations where it is useful to be able to determine the source code provenance of a binary. While previous work has either focused on computing binary-to-binary similarity or source-to-source similarity, BinPro is the first work we are aware of to tackle the problem of source-to-binary similarity. BinPro can match binaries with their source code even without knowing which compiler was used to produce the binary, or what optimization level was used with the compiler. To do this, BinPro utilizes machine learning to compute optimal code features for determining binary-to-source similarity and a static analysis pipeline to extract and compute similarity based on those features. Our experiments show that on average BinPro computes a similarity of 81% for matching binaries and source code of the same applications, and an average similarity of 25% for binaries and source code of similar but different applications. This shows that BinPro's similarity score is useful for determining if a binary was derived from a particular source code.

==> compilerOptimization.tex <==
\subsection{Handling other optimizations}
\label{sec:compilerOptimization}

\iffalse
\begin{enumerate}
\item Function Inlining
\item number of parameters
\item number of conditional branches
\item detection phase: additional string constants and library calls
\end{enumerate}
\fi


% this sentence says nothing.
%While BinPro is able to correctly match many binary code functions with the correct source code function and determine the absence of a backdoor, there are still anywhere from 10-35\% of functions where it is unable to do.  The main reason for this is benign compiler optimizations.  Since static compilers cannot use dynamic profiles to guide when to apply optimizations, they often must rely on complex algorithms to determine optimizations should be applied.  

%With the exception of inlining, we found it ineffective to try to predict when these other optimizations will occur.  

% this paragraph is also not saying very much
%Two design features in BinPro enable it to achieve matches despite compiler optimizations.  First, function matching allows functions with minor differences to match during function matching.  Second, BinPro only checks suspicious features indicative of a backdoor during equivalence checking.  For example, a commonly applied optimization that BinPro does not try to predict is loop unrolling, which will increase the number of conditional branches used in the CFG feature.  However, such an optimization does not introduce new logical paths into the function, and cannot be used to insert a backdoor into a binary, so BinPro does not need to account for it.

%However, this optimization has only a minor effect on the final result of BinPro since it is only used during the refinement phase.  

Compilers may also perform library call substitutions that replace some standard library calls with more efficient versions if the call-site arguments permit it.  While these differ widely from compiler to compiler, and thus are a poor target for training unless one has access to the compiler itself (something BinPro does not assume), they are fairly easily recognizable by a human auditor, as they are almost universally applied to standard library functions and a human who understands the semantics of the library calls would be able to easily determine their equivalence (i.e. replacing {\tt printf} with {\tt puts} or {\tt vsprintf}).  Thus, BinPro can be configured with a whitelist of such substitutions.  Once the auditor notices a compiler making such substitutions, they can add the substitution to BinPro's whitelist and run BinPro again, which prevents it from incorrectly marking these substitutions as unsafe.  A similar whitelist also exists for compiler-inserted functions  such as \texttt{\_\_stack\_chk\_fail}, which GCC inserts to detect stack overflow.

We found that string constants, FCG callers and FCG callees are rarely modified by compiler optimizations, making them reliable for function matching.  As we detail in Section~\ref{sec:machineLearningImplementation}, these three features are given the heaviest weight factors by our machine learning algorithm.  The major case where compilers insert strings are with pre-processor defined strings, such as {\tt \_\_LINE\_\_} or {\tt \_\_FILE\_\_}.  Another more obscure case was where format strings that contained a substitution that could be statically resolved (i.e. {\tt sprintf(str, "\%d", 5)}) might be performed at compilation time.  While it might be possible to check some pre-processor inserted strings, in general, these string substitutions are difficult to whitelist as the inserted string can be very dependent on the environment where the binary was compiled (i.e. the date or compiler version).  As a result, BinPro does not currently whitelist any compiler-generated string constants.

%Only a few compiler optimizations affect these features as previously discussed in Section~\ref{sec:problemDefinition-optimizations}.  Out of these, the largest effect is library call substitutions.  




%\textbf{Other minor optimizations:} Compilers also optimize control-flow basic blocks to improve the performance of the execution. For instance, loop unrolling optimization may completely unroll loop and we see a mis-match between the CFG derived from the source code and binary. This affects \(num\_cond\_br\) features and inaccurately calculate the similarity cost. However, we are not heavily dependent on this feature and only used as a conflict resolution among \textit{May-Be-Matched} functions.


% TODO: Put this inside evaluation section. 
%Even then, we are still able to accurately determine \(num\_parameters\) with approximately 65\% among the 10 applications. 

%Lastly, we show how feature 1 and 3 are affected because of compiler optimizations. These features are used for determining similarity and differences among functions. Compilers rarely adds string constants in the binary, which does not exist in the source code. For example, the binary may  contains additional string constant such as date at which the binary was compiled on, path of a source file, and other metadata. These information are derived and injected in the binary during the compilation process and this is why we do not see in the source code. These additional string constants in the binary gets caught during the detection phase even though these strings are benign and not malicious. Such string constants sparsely occurs and we observed that they could be white listed to improve the backdoor detection, and we leave it for future work. 
%Even though we don't deal with it, you can suggest a possible solution.  For example, do you think we could whitelist these?  If so, you should say that we feel these could be white listed, and leave it for future work.

%On the other hand, compilers often substitute one library calls with other one. For example, \(printf\) gets substituted with \(puts\) as we see in the \texttt{init()} function in PlayGame's FCG. This affects the strict matching phase where we determine the differences. To mitigate this issue, we added a whitelist of benign transformations of substitution of library calls made by the compiler, and the Table~\ref{table:substitution} presents this whitelist. 


%Ideally our tool should be able to match all the functions from the binary to the source code functions if the compiler optimization is turned off. This means that any change in the binary may that be addition or removal of functionality is distinguishable and the tool is able to detect it fairly easily. However, in real world scenario the binaries used in the production uses some levels of compiler optimization. 



%\textbf{Function Inlining:} This optimization is very critical because some functions are removed from the binaries. This removal causes the addition of features to the other set of functions. More precisely, a same function in the binary and the source code will appear differently; features in the binary may have additional library calls, caller and callee nodes, CFG etc. This optimization makes the matching phase non-trivial to handle. 
%
%We extract features 8$-$15 (listed on Table~\ref{table:featureSet}) from the source code for each function. These features are used to predict whether the function is inlined or not. We create a vector of these features for every function and label them as \textit{Inlined} or \textit{Not-Inlined} based on the ground truth. A ground truth is determine by compiling the source code with gcc with different optimization levels (\texttt{-O2}, \texttt{-O3}), where the debug flag is turned on. A debugged version of the binary produces debugging information such as DWARF \cite{GCC}. We use Dwarfdump \cite{Dwarfdump} tool to get the list of functions in the binary that are inlined based on the compiler debug information.   
%
%We create a training set comprises of both the \textit{Inlined} and \textit{Not-Inlined} feature vector on all 10 different applications varies in size and complexity, namely, Proftpd, Apache, Busybox, Bind, Mongoose, Lighttpd, Dropbear, OpenSSH, Transmission and OpenVPN. The training set is split in to 50\% \textit{Inlined} and 50\% \textit{Not-Inlined} so that it is not heavily biased on either class. Using this training set we train on Alternating Decision Tree (ADTree) machine learning algorithm \cite{ADTree} using Weka \cite{weka} framework. 
%
%Using this trained ADTree matching learning model, we predict whether a function is inlined or not. During the features extraction stage, we use this model to predict every functions in the source code. If ADTree predicts a function to be inlined, then all its features are copied to its respective caller. Moreover, we add additional edges to the FCG from the caller for the inlined node to callee of the same node. This gives an impression as if the function is inlined. For example we can see from the call graphs of PlayGame, \texttt{init()} is inlined in the binary and \texttt{printf()} library call is transitioned to \texttt{main()}. We do not remove the inlined function from the FCG of the source code because we know that machine learning may mis-predict. If we inline a function, which is not suppose to be inlined, the matching phase still find a correct match as the inlined function is not removed. \\












==> limitations.tex <==
\section{Limitation and Future Work}
\label{sec:limitation}

==> problemDefinition.tex <==
\section{Problem definition}
\label{sec:Preliminaries}

\subsection{Backdoors}
\label{sec:problemDefinition}
Backdoors are intentionally inserted hidden functionality that allows a malicious attacker to bypass security mechanisms.  While there are innumerable ways that attackers can implement a backdoor, we can informally classify all backdoors into two broad categories -- those that add additional functionality to bypass security mechanisms, and those that weaken existing security mechanisms so that they can be bypassed.  The former are what are traditionally considered backdoors, and include functionality such as a hard-coded passwords, ``easter eggs'' that are triggered by unusual or invalid inputs or code that surreptitiously connects to a remote service to retrieve commands.  The latter type of backoors are essentially ``vulnerabilities'', and only differ from traditional vulnerabilities in that they have been intentionally, as opposed to accidentally, inserted.  A good example that illustrates this difference is the pair of backdoors recently discovered in Juniper ScreenOS Firewall products~\cite{juniper-backdoor}, which are used by governments, banks and telecommunications providers around the world.  One backdoor is a hardcoded password that allows an attacker to gain administrative access to the firewall.  The other backdoor was a weakened random number generator used to generate keys for encryption of VPN traffic, that, when combined with another information leakage vulnerability, can allow an attacker to predict future keys.  While the former is clearly intentionally inserted, the main reason that the latter is suspected to be a backdoor stems from leaked NSA documents describing secret exploit capability against ScreenOS~\cite{nsa-screenos}.  

In this paper, we focus on the former type of ``additive'' backdoor for several reasons.  First, additive backdoors generally have the potential to do more damage than ``vulnerability'' backdoors.  In the Juniper example, the vulnerability backdoor only provided passive decryption capability, while the additive backdoor does that and more by giving the attacker full administrative capability.  Second, additive backdoors are easier to detect during a source code audit, while vulnerability backdoors are extremely difficult to detect, as they are no different from other vulnerabilities and bugs in software, which are notoriously hard to detect.  As a result, an attacker is more likely to insert additive backdoors only into the binary, since even if inserted into source code, vulnerability backdoors have a lower chance of being discovered.  For simplicity, the rest of the paper will refer to additive backdoors simply as ``backdoors'', and vulnerability backdoors as ``vulnerabilities''.

We survey several recently documented backdoors to understand how they are implemented.  While there haven't been a large number of publicly documented cases, the similarity between them give us confidence that most modern backdoors should  have similar characteristics.  In the ProFTP backdoor~\cite{proftp-backdoor} a secret FTP command (\texttt{"ACIDBITCHEZ"}) was implemented that when called by the attacker, would grant access to a root shell.  The D-Link~\cite{dlink-backdoor} and Juniper~\cite{juniper-backdoor}, and Fortinet~\cite{fortinet-backdoor} backdoors all used various long, hard-coded passwords, that would grant the attacker administrative access.  In the Linksys/Netgear~\cite{linksys-backdoor} backdoor, the affected device listened in on a secret port that would execute administrative commands without a password.  

In all these cases, the attacker is needs to make the backdoor stealthy, so that it is unlikely to be triggered by accident.  Thus, the backdoor must either be guarded by a check that only passes under some unusual input, or it must automatically operate and accept remote commands.  We thus formalize our backdoor threat model as either: 1) a new function is added to the application, 2) new function calls or library calls are added to an existing function, or 3) a new code path guarded by a long string or unusual set of constants is inserted.  These three cases map to code features such as function calls and control-flow checks on strings and constants, which we call {\em suspicious features} since they are necessary for a backdoor to exist.

Na\"{i}vely, one could imagine simply searching a binary for all sections of code that contain such features.  However, this would result in numerous false alarms since these features all occur abundantly in benign code.  The critical difference is that these features are malicious when they have been inserted into a binary and do not appear in the corresponding source code.  As a result, BinPro screens binaries by comparing them against source code and only flagging these suspicious features when they appear in a binary and can't be matched in the source code.

%Proving equivalence between two programs is equivalent to the halting problem, and is thus undecidable.  For the same reason, it is difficult to prove that compilers produce binary code that is equivalent to the input source code~\cite{necula_translation_2000,leroy_formal_2009}.  Rather than try to prove equivalence between a binary and source code, BinPro instead aims for a weaker property, which we call {\em Binary Backdoor Accountability}.  Binary backdoor accountability aims to identify the functions in a binary that are accounted for by functions in some corresponding source code. The binary functions that are accounted for by the source code functions must not contain a backdoor. This means that if a function in a binary contains a backdoor, BinPro must not be able to identify it's equivalent function in the source code. 


%DL remove the mapping to coverage problem -- not really relevant
%We define the call graph of binary $\mathbb{B}$ as accountable by the call graph of source code $\mathbb{S}$ iff every function $b$ in $\mathbb{B}$ $matches$ a non-empty set of functions $s$ in $\mathbb{S}$.  The inverse is not true -- functions in $\mathbb{S}$ do not have to match a function in $\mathbb{B}$ because source code can be present but not included into the final binary or the compiler may optimize some source code functions away.  

%In the above formulation, we define $match$ as a function that will return true if $b$ is produced from $s$ under benign compilation, but false if a backdoor is inserted into $b$ that is not present in $s$.  
%We can categorize backdoors in two types, on a high-level: 1) backdoors that add functionality in the binary, which we call \textit{zero-door} backdoor, and 2) backdoors that weaken or break existing functionality, either by introducing or exploiting vulnerabilities. 
%We define a backdoor inserted into the binary as malicious code that: 1) specifies malicious functionality that is not present in the source code and 2) that malicious functionality should be triggered only under very specific circumstances so as to remain stealthy.  
%In some cases, the backdoor could be a large amount of functionality, such as making additional network and file system calls, features found in many remote access tools (i.e. RATS)~\cite{rats}.  These give a remote attacker access to nearly unlimited functionality on the victim machine.  In other cases, the additional functionality could be as little as an additional code path that allows an attacker to bypass authentication with a hardcoded password or secret keyword, such as that found in various well-documented backdoors~\cite{dlink-backdoor, juniper-backdoor, fortinet-backdoor}.  In this case, the attacker only has access to legitimate functionality in the binary, but in many cases this is still enough functionality to do a great deal of damage.  As a result, we focus \textit{zero-door} type of backdoor, which we believe that a great majority of backdoors will fall in this category. We thus formalize our zero-door backdoors threat model that add new functionality: 
%1) new function definition,
%2) new code paths guarded by hardcoded strings or constants are inserted to make them stealthy,
%3) new function call or library call. 
%Hence, binary backdoor accountability claims that the two functions that are equivalent by not containing a zero-door backdoors. It does not mean that these two functions do not contain bugs or vulnerabilities.   
%
%We note that our backdoor model excludes backdoors that are built around vulnerabilities, as these do not need to insert new functionality.  For example, if an attacker inserts a memory corruption vulnerability that they can later exploit to inject new code or perform a return-oriented-programming attack~\cite{shacham_geometry_2007}, then the new functionality does not appear in the binary, but is instead injected at exploit time.  Since binary backdoor accountability is a static analysis technique, it cannot analyze new dynamically injected functionality. 

\subsection{Assumptions}
\label{sec:assumptions}
We make several assumptions in this work.  First, we do not assume the presence of source code symbols in the binary, however, we do assume that it can be reliably disassembled using a tool such as IDAPro~\cite{ida}.  While it is possible to produce binaries that would defeat IDAPro, since the binary is meant to be benign, a binary that contains obfuscated code is likely to draw suspicions in it of itself.  

%We concede that it may be possible for an adversary to obfuscate their backdoor so that it also happens to disassemble to normal-looking code (for example, by overlaying 2 different instruction streams over the same binary values).  However, this requirement raises the level of difficulty for the attacker considerably.

Second, we do not assume we have access to the build infrastructure or the exact compiler used to build the binary.  However, we do assume that we are able to pass all the source code through our analysis tools, meaning that they are in some dialect of C or C++ that we can parse.  For now, we also assume access to the values used in processor directives (i.e. \texttt{\#ifdef}) and include files so as to avoid undefined or incorrectly defined symbols in our code parser, which was derived form a standard C/C++ compiler.  This artifact can be overcome by modifying the front-end of our tool to ignore undefined symbols and accept mismatched types, which we plan to do for future work.


\myfigwide{WorkFlow.png}{High-level work flow of BinPro}{fig:workFlow}{0.9}{-20pt}
%\begin{figure*}[tb]
%	\begin{center}
%		\includegraphics[scale=0.65]{WorkFlow.png}
%	\end{center}
%	\caption{High-level work flow of BinPro}
%	\label{fig:workFlow}
%\end{figure*}
\subsection{Compiler optimizations}
\label{sec:problemDefinition-optimizations}
The main difficulty with binary backdoor screening is separating differences between a binary and its source due to backdoors from those due to compiler optimizations.  Compiler optimizations obscure the relationship between the binary and source code, making it challenging to correctly screen code.  In general, proving that compilers produce binary code that is equivalent to the input source code is the same as solving the halting problem, and is thus undecidable~\cite{necula_translation_2000,leroy_formal_2009,wang_towards_2013}.  However, BinPro need not check for complete equivlance.  Instead, BinPro only has to screen the binary against the source for extra suspicious code features as those features are required to implement a backdoor.  Because the suspicious code features consist of references to string and integer constants or calls to local and library functions, BinPro can abstract away local and instruction-level compiler optimizations such as loop unrolling, common subexpression elimination or opcode substitution.  



% too early, haven't talked about matching functions
%Optimizations could cause BinPro to incorrectly match a binary functions with a different source code function, which as a result, will cause BinPro to incorrectly flag differences as unsafe.  Even if BinPro does correctly match the function, compiler optimizations can still alter suspicious features and lead BinPro to incorrectly suspect a backdoor.

%determine if a particular backdoor feature in a binary can be correctly matched to a feature in the source code, or whether it has been added by an adversary.  


Instead, BinPro need only account for optimizations that can modify the suspicious features.  The main compiler optimization that can do this is function inlining, where a compiler may insert a function into the body of its caller.   As a result, the suspicious features of the callee (such as callees, string constants and integer constants) will be moved into the caller.  Since every function could potentially be inlined, this would seem to present an nearly infinite number of possibilities.  However, the key observation that BinPro leverages is that compilers are generally conservative and only apply optimizations when they are safe and confer an advantage.  This conservative bias dictates that there is some similarity in the rules governing optimizations across compilers.  BinPro takes advantage of this to apply machine learning on the code features that influence inlining and build a model that allows it to predict when function inlining will occur, allows BinPro to account for the effects of function inlining.

%Even without access to the exact rules used to compile the binary, BinPro is able to approximate them using machine learning and predict where optimizations are likely to occur.  

%This allows BinPro to narrow the scope of features in the source code that a suspicious feature in a binary could match to, allowing it to perform binary screening with greater accuracy.  


%For example, function inlining is an optimization where a compiler may insert a function into the body of its caller.  As a result, the suspicious features of the callee will now appear in the caller.  Functions can be recursively inlined into their callers, resulting in a myriad of code feature combinations that could appear in the top-level caller.  Other optimizations, such as branch combining and expression simplification can change the number of control-flow statements and the values checked in those statements.


% we don't really deal with these so don't put them in the problem definition.
%In addition to inlining, other optimizations compilers can perform are function substitution for common library calls (i.e. \texttt{printf} to \texttt{puts}), inserting string constants (i.e. macros such as {\tt \_\_FUNC\_\_} or {\tt \_\_FILE\_\_}), inserting helper function calls (i.e. \texttt{\_\_stack\_chk\_fail} by GCC to detect stack overflow) or local optimizations control-flow graph (CFG) optimizations (i.e. loop unrolling).  


%\iffalse
%
%Fortunately, many optimizations are orthogonal to backdoor screening as they do not introduce or remove library, nor do they affect hardcoded strings or constants used in a binary.
%
%
%However, there are several that do, which we briefly outline here.
%
%\scbf{Inlining} This optimization moves a callee function into the body of a caller function, essentially removing the callee from the binary.  In addition, a new function will be created that will be a mix of the features of both the original callee and caller.  Inlining makes binary backdoor screening hard because two or more functions in the source code must be properly matched to a single function in the binary.  The handling of arbitrary inlining by BinPro is a distinguishing characteristic over previous work~\cite{pewny_crossarchitecture_2015,eschweilersebastian_discovre_2016}, which will return incorrect results if inlining occurs
%
%\scbf{Library call substitution} Compilers may have standard library-specific optimizations that substitute library calls for a more efficient version under certain circumstances.  In many of these cases, these library calls may make different system calls. Binary backdoor screening must properly disambiguate these benign optimizations from modifications that would result from an addition of a backdoor in the binary.
%
%\scbf{Local optimizations} Compilers also optimize control-flow basic blocks to improve the performance of the execution. For example, optimizations such as loop unrolling may significantly change the structure of the control-flow graph.  In addition, register allocation optimizations can obscure the number of parameters passed to a function at certain call sites if the compiler determines that the appropriate argument is already in the appropriate register.  
%
%\scbf{String modification} Compilers may insert new string constants in the compilation process (i.e. standard pre-defined macros such as {\tt \_\_FUNC\_\_} or {\tt \_\_FILE\_\_}), as well as modify existing ones (for example, perform statically resolvable string substitutions for format string functions).  
%
%\scbf{Compiler-inserted functions}  Compiler will sometimes insert their own calls to helper functions.  For example, GCC will insert calls to \texttt{\_\_stack\_chk\_fail} to detect stack overflow.  These functions appear in the binary but not in the source code.  BinPro will flag these functions as unaccounted for since they do not have a source code equivalent.  However, they are easily recognizable and can be easily white listed by users.
%
%
%
%
%
%\section{Preliminaries}
%\label{sec:problemDefinition}
%
%\subsection{Problem definition}
%Proving equivalence between two program is equivalent to the halting problem, and is thus undecidable.  For the same reason, it is difficult to prove that compilers produce binary code that is equivalent to the input source code~\cite{necula_translation_2000,leroy_formal_2009}.  Rather than try to prove equivalence between a binary and source code, BinPro instead aims for a weaker property, which we call {\em binary backdoor accountability}.  binary backdoor accountability aims to identify the functions in a binary that are accounted for by functions in some corresponding source code. 
%
%%DL remove the mapping to coverage problem -- not really relevant
%We define the call graph of binary $\mathbb{B}$ as accountable by the call graph of source code $\mathbb{S}$ iff every function $b$ in $\mathbb{B}$ $matches$ a non-empty set of functions $s$ in $\mathbb{S}$.  The inverse is not true -- functions in $\mathbb{S}$ do not have to match a function in $\mathbb{B}$ because source code can be present but not included into the final binary or the compiler may optimize some source code functions away.  
%
%In the above formulation, we define $match$ as a function that will return true if $b$ is produced from $s$ under benign compilation, but false if a backdoor is inserted into $b$ that is not present in $s$.  We define a backdoor inserted into the binary as malicious code that: 1) specifies malicious functionality that is not present in the source code and 2) that malicious functionality should be triggered only under very specific circumstances so as to remain stealthy.  In some cases, the backdoor could be a large amount of functionality, such as making additional network and file system calls, features found in many remote access tools (i.e. RATS)~\cite{rats}.  These give a remote attacker access to nearly unlimited functionality on the victim machine.  In other cases, the additional functionality could be as little as an additional code path that allows an attacker to bypass authentication with a hardcoded password or secret keyword, such as that found in various well-documented backdoors~\cite{dlink-backdoor, juniper-backdoor, fortinet-backdoor}.  In this case, the attacker only has access to legitimate functionality in the binary, but in many cases this is still enough functionality to do a great deal of damage.  While we do not claim that these two classes of backdoors are exhaustive, we believe that a great majority of backdoors will fall into one of these cases.  We thus formalize our backdoor threat model based on these two classes where either: 1) new function calls that eventually lead to system calls are inserted, or 2) new code paths guarded by hardcoded strings or constants are inserted to make them stealthy.
%
%We note that our backdoor model excludes backdoors that are built around vulnerabilities, as these do not need to insert new functionality.  For example, if an attacker inserts a memory corruption vulnerability that they can later exploit to inject new code or perform a return-oriented-programming attack~\cite{shacham_geometry_2007}, then the new functionality does not appear in the binary, but is instead injected at exploit time.  Since binary backdoor accountability is a static analysis technique, it cannot analyze new dynamically injected functionality.
%
%\subsection{Assumptions}
%\label{sec:assumptions}
%We make several simplifying assumptions in this work.  First, while we do not assume access to compilation symbols, we do assume that it can be reliably disassembled using a tool such as IDAPro~\cite{ida}.  While it is possible to produce binaries that would defeat IDAPro, since the binary is meant to be benign, a binary that contains obfuscated code is likely to draw suspicious in it of itself.  We concede that it may be possible for an adversary to obfuscate their backdoor so that it also happens to disassemble to normal-looking code (for example, by overlaying 2 different instruction streams over the same binary values).  However, this requirement raises the level of difficulty for the attacker considerably.
%
%Second, while we do not assume we have access to the build infrastructure, we do assume that we are able to pass all the source code through our analysis tools, meaning that they are in some dialect of C or C++ that we can parse.  For now, we also assume access to the values used in processor directives (i.e. \texttt{\#ifdef}) and include files so as to avoid undefined or incorrectly defined symbols during our parser, which was derived form a standard C/C++ compiler.  However, this is an implementation artifact as one could also modify the front-end of our tool to ignore undefined symbols and accept mismatched types, which we plan to do for future work.
%
%\subsection{Compiler optimizations}
%\label{sec:problemDefinition-optimizations}
%One of the main difficulties with determining binary backdoor accountability is the code transformations compilers apply to optimize the compiled binary.  Fortunately, many optimizations are orthogonal to binary backdoor accountability as they do not introduce or remove system calls, nor do they affect hardcoded strings or constants used in a binary. However, there are several that do, which we briefly outline here.
%
%\scbf{Inlining} This optimization moves a callee function into the body of a caller function, essentially removing the callee from the binary.  In addition, a new function will be created that will be a mix of the features of both the original callee and caller.  Inlining makes binary backdoor accountability hard because two or more functions in the source code must be properly matched to a single function in the binary.  The handling of arbitrary inlining by BinPro is a distinguishing characteristic over previous work~\cite{pewny_crossarchitecture_2015,eschweilersebastian_discovre_2016}, which will return incorrect results if inlining occurs
%
%\scbf{Library call substitution} Compilers may have standard library-specific optimizations that substitute library calls for a more efficient version under certain circumstances.  In many of these cases, these library calls may make different system calls. binary backdoor accountability must properly disambiguate these benign optimizations from modifications that would result from an addition of a backdoor in the binary.
%
%\scbf{Local optimizations} Compilers also optimize control-flow basic blocks to improve the performance of the execution. For example, optimizations such as loop unrolling may significantly change the structure of the control-flow graph.  In addition, register allocation optimizations can obscure the number of parameters passed to a function at certain call sites if the compiler determines that the appropriate argument is already in the appropriate register.  
%
%\scbf{String modification} Compilers may insert new string constants in the compilation process (i.e. standard pre-defined macros such as {\tt \_\_FUNC\_\_} or {\tt \_\_FILE\_\_}), as well as modify existing ones (for example, perform statically resolvable string substitutions for format string functions).  
%
%\scbf{Compiler-inserted functions}  Compiler will sometimes insert their own calls to helper functions.  For example, GCC will insert calls to \texttt{\_\_stack\_chk\_fail} to detect stack overflow.  These functions appear in the binary but not in the source code.  BinPro will flag these functions as unaccounted for since they do not have a source code equivalent.  However, they are easily recognizable and can be easily white listed by users.
%
%
%
%% This affects \(num\_cond\_br\) features and inaccurately calculate the similarity cost. However, we are not heavily dependent on this feature and only used as a conflict resolution among \textit{May-Be-Matched} functions.
%
%


%
%
%We assume that the given binary is stripped, i.e. it does not contain any debug symbols. We further assume that the binary is not packed and is compiled with C/C++ programming languages. While packed binaries is beyond the scope of this paper, several work have been proposed that deals with the unpacking and are complementary to our work [REFs]. 
%
%The preprocessor directives, such as \texttt{\#ifdef} and \texttt{\#include} in the source code, have a significant effect on the compiled binary. Depending on the directive defined in the argument used by the compiler, for example with \texttt{-D} flag in \texttt{gcc}, certain functions or code will be added or removed. Moreover, there could be many header files with the same name in the source code. These duplicate header files are resolved by the \texttt{Makefile} depending on the preprocessor directives. Thus, we assume that the make infrastructure, such as \texttt{Makefile}, is included in the source code to resolve preprocessor directives and duplicate header files. 
%
%Having said that, we do not assume anything about the compiler the binary was compiled with and the optimization level used. One such optimization is function inlining where an inlined function's body is copied to the caller function. This incurs a huge challenge when dealing with binary to source code comparison, where other previous works do not address solutions to this problem. 



%Due to globalization and cost, software development is out-sourced to other countries. We rely on software components that are not implemented by ourselves; rather we use third party software or libraries, for instance open-source project or a commercially available product. Hence, there is a possibility of software supply chain attach, where software that comes from a trusted source has malware incorporated into the binary at some point, as we saw with \texttt{Linux/Cdorkedbackdoor.A} backdoor in Apache web server [REF].
 
%We informally define binary provenance problem as ensuring whether a binary matches the source code provided, and there are no additional functionalities such as backdoors in them. In this problem setting we are provided with an untrusted binary and a benign source code. The objective is to determine the similarities and dissimilarities between the binary and source code. In this context, similarity means that the binary is derived or compiled from the given source code, whereas dissimilar binary means that there exists additional functionality in the binary, which is not in the source code. 

%You need some discussion here about what a backdoor is, and why you focus only on these two very specific types of backdoors. You should gracefully concede that there could be and are other types of backdoors.

%Of course, executing unknown code has several security implications; among others it in- volves the question whether the executable has some un- documented, unwanted, or hidden functionality [35]. Pur- posefully (or even unintentionally) the program could for example have an undocumented account that is only avail- able upon specific conditions [2], or offer another kind of remote access to an adversary [3?5].

%[35] ->  K. Thompson. Reflections on trusting trust. Commun. ACM, 27(8), Aug. 1984.
%[2] -> ProFTPD Backdoor Unauthorized Access Vulnerability, 2010. http://www.securityfocus.com/bid/45150.
%[3] Backdoor Found In Arcadyan-based Wi-Fi Routers, 2012. http://it.slashdot.org/story/12/04/26/ 1411229/backdoor-found-in-arcadyan-based-wi- fi-routers.
%[4] RuggedCom - Backdoor Accounts in my SCADA network? You don?t say..., 2012. http: //seclists.org/fulldisclosure/2012/Apr/277.
%[5] Samsung printers contain hidden, hard-coded management account, 2012. http://www.zdnet.com/ samsung-printers-contain-hidden-hard-coded- management-account-7000007928/.

%A backdoor is an undisclosed and undocumented secret method or program to bypass certain security measures based on some triggers to perform malicious activity. Security measures a backdoor bypasses include authentication or permission based access control. Backdoor are usually used for acquiring unauthorized access to a system using a hardcoded password [REFs], secretively downloading remote code [REF], and stealing information, such as obtaining cryptographic keys. Many recent backdoors, for instances Dlink [REF], Juniper Network [REF] and Fortinet [REF], are implemented to contain hardcoded string. Furthermore, there are other types of backdoors, which uses library/system calls for their malicious activity, such as port-knocking [REF], stealing information by reading a file. Thus, our threat model consists of backdoors of the following two types:
%
%\begin{enumerate}
%\item \textit{Hardcoded-password.} A binary contains additional string constant(s)  compared to the source code. See Listing XX for code snippet for example. 
%\item \textit{Additional functionality.} A binary contains additional library call(s), for example \texttt{open(...)} to open a file. This is a generic type of backdoor that requires system/library call to enable remote control, steal and leak information, or download other code and execute it. %, or more complex port-knocking backdoor [REF].  
%\end{enumerate} 
%
%We believe that there are other types of backdoors, which do not fall in one of the two categorizes mentioned above. For example, Adam and Moti introduced asymmetric backdoors that can only be used by the backdoor developer, even if the implementation is publicly available [REF]. \\ \\
% REF -> Proceedings of Advances in Cryptology: Crypto '96
%  ->  "wired.com: "How a Crypto ?Backdoor? Pitted the Tech World Against the NSA" (Zetter) 24 Sep 2013" http://www.wired.com/threatlevel/2013/09/nsa-backdoor/all/

%I think you need to add some discussion about the assumption that we can use the make infrastructure to the problem definition.

%Moreover, we do not assume anything about the compiler the binary was compiled with and the optimization level used. This is to say that the compiler or the build environment used by the source code developers is not provided. Therefore, our test dataset described in section~\ref{sec:evaluation} to evaluate BinPro is compiled with GNU \texttt{gcc} and Intel \texttt{icc}, with all the optimization levels. 









%The problem of determining binary backdoor accountability is similar to the problem of determining if $\mathbb{S}$ is a covering graph of $\mathbb{B}$ with some key differences.  First, Second, most graph matching problems assume that the labels on the nodes are unambiguous -- i.e. the set of nodes in $\mathbb{S}$ that match any particular node in $\mathbb{B}$ is clearly defined.  This is not the case for binary backdoor accountability because the complication process obscures the relationship between nodes in $\mathbb{S}$ and $\mathbb{B}$.  For example, local compiler optimizations may change code features so that a function's binary version does not exactly match its source version.  In addition, inter-procedural optimizations may inline some source functions into other functions so that the nodes in the set $s$ may be a refinement of the nodes in node $b$.  Finally, a single function $b$ may be defined multiple times in source code $\mathbb{S}$ under different target-specific subdirectories.

%\fi

